Extended Formulations via Decision Diagrams

We propose a general algorithm of constructing an extended formulation for any given set of linear constraints with integer coefficients. Our algorithm consists of two phases: first construct a decision diagram $(V,E)$ that somehow represents a given $m \times n$ constraint matrix, and then build an equivalent set of $|E|$ linear constraints over $n+|V|$ variables. That is, the size of the resultant extended formulation depends not explicitly on the number $m$ of the original constraints, but on its decision diagram representation. Therefore, we may significantly reduce the computation time for optimization problems with integer constraint matrices by solving them under the extended formulations, especially when we obtain concise decision diagram representations for the matrices. We can apply our method to $1$-norm regularized hard margin optimization over the binary instance space $\{0,1\}^n$, which can be formulated as a linear programming problem with $m$ constraints with $\{-1,0,1\}$-valued coefficients over $n$ variables, where $m$ is the size of the given sample. Furthermore, introducing slack variables over the edges of the decision diagram, we establish a variant formulation of soft margin optimization. We demonstrate the effectiveness of our extended formulations for integer programming and the $1$-norm regularized soft margin optimization tasks over synthetic and real datasets.

==> experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}
We show preliminary experimental results on artificial and real large data sets. 
The tasks are, the set covering problem (see, e.g., \citet{williamson-shmoys:book11}), an integer programming task, and 
the $1$-norm regularized soft margin optimization, a linear programming task, as in (\ref{prob:softmargin_primal}).
Our experiments are conducted on a server with 2.60 GHz Intel Xeon Gold 6124 CPUs and 314GB memory.
We use Gurobi optimizer 9.01
\footnote{Gurobi Optimization, Inc.,\url{http://www.gurobi.com} }, an state-of-the-art commercial LP solver.
To obtain NZDD representations of data sets, we apply the procedure described in Section \ref{sec:construction}.
The details of preprocessing of data sets and NZDD representations are shown in Appendix.

\subsection{Integer programming(IP)}
First, we apply our extended formulation (\ref{prob:lin_const_opt}) to the set covering problem~\citep{}, an integer programming tasks.
We use real datasets tested in the paper of \citet{cormode-etal:cikm10}, 
which are found in Goethal's web page~\citep{goethals:web} and 
in the UCI Machine Learning Repository~\citep{uci-ml}. 
Here, our intention on these experiments is not to compare the state-of-the-art set covering solvers (e.g.,\citet{cormode-etal:cikm10}),
but to confirm advantages to off-the-shelf IP solvers on general IP data sets. 
So, we apply the Gruobi optimizer to the standard IP formulation of the set covering 
and our extended formulation for the set covering, respectively.
The results are summarized in Figure~\ref{fig:setcover}. 
Our method consistently improve both computation time and often reduce memory usage. 

\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_time_setcover.pdf}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_memory_setcover.pdf}
        \caption{Comparison of computation times and maximum memory consumption 
        for real datasets of set covering problems. The y-axes are shown in the logarithmic scale.}
        \label{fig:setcover}   
    \end{center} 
\end{figure}


\iffalse
\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of computation times for real data sets.}
        \label{tab10}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{Computation time(sec.)} \\ \hline
            data set    & naive LP & proposed\\ \hline
            chess       &     $0.15$ & $0.1$ \\
            connect     &     $7.26$ & $3.82$ \\
            mushroom    &     $0.15$ & $0.01$  \\
            pumsb       &     $14.5$ & $14.23$  \\
            pumsb\_star &    $10.89$ & $8.64$ \\ \hline
        \end{tabular}
    \end{center}
\end{table}

\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of maximum memory consumption for real data sets.}
        \label{tab9}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{memory(MB)} \\ \hline
            data set    & naive LP & proposed\\ \hline
            chess       &     $26$ & $22$ \\
            connect     &    $656$ & $192$ \\
            mushroom    &     $35$ & $13$  \\
            pumsb       &    $504$ & $544$  \\
            pumsb\_star &    $348$ & $359$ \\ \hline
        \end{tabular}
    \end{center}
\end{table}
\fi




\subsection{$1$-norm soft margin optimization}

We compare the following methods.
\begin{description}
    \item[LP] 
    We naively apply the LP solver to solve problem (\ref{prob:softmargin_primal}).
    \item [LPBoost] 
    LPBoost\citep{demiriz-etal:ml02} is a standard method for solving (\ref{prob:softmargin_primal}).
    LPBoost is a "column-generation" type medhod, i.e., 
    it solves the dual subproblems of (\ref{prob:softmargin_primal}) iteratively by adding constraints.
    \item[Our method]...
\end{description}



\subsubsection{Experiments on Artificial Data Sets}
We use a class of artificial data sets that have small NZDD representations when the samples are large. 
Our artificial data sets are made by a simple linear threshold function over the domain $\{0,1\}^n$ for some positive integer $n$.
First, we choose $m$ instances in $\{0,1\}^n$ uniformly randomly without repetition. 
Then we consider the following linear threshold function $f(\vecx)=\sign(\sum_{j=1}^k x_j - r+ 1/2)$, 
where $k$ and $r$ are positive integers such that $1\leq r\leq k\leq n$).
That is, $f(x)=1$ if and only if at least $r$ of the first $k$ components are $1$. We call this $r$-of-$k$ threshold function.
Each label of the instance $\vecx\in\{0,1\}^n$ is labeled by $f(\vecx)$. It can be easily shown that 
the whole labeled $2^n$ instances of $f$ is represented by an NZDD (or ZDD) of size $O(kr)$, 
which is exponentially small w.r.t. the sample size $m=2^n$. 
We fix $n=20$, $k=10$ and $r=5$. Then we use $m \in \{1*10^5,2*10^5...,10^6\}$.

\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_time_artificial.pdf}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_memory_artificial.pdf}
        \caption{Comparison of computation times and maximum memory consumption 
        for artificial data sets. 
        Results for naive LP w.r.t. $m\geq 6*10^5$ are omitted since it takes more than $1$ day.}
        \end{center}
    
\end{figure}

\iffalse
\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of computation times for artificial data sets.}
        \label{tab2}
        \begin{tabular}{|l||r|r|r|r|r|r|r|} \hline 
            & \multicolumn{6}{|c|}{Computation time (sec.)} \\ \hline
            Sample size ($m$) & naive LP & LPBoost &   ERLP & NZDD-LP & NZDD-LPBoost & NZDD-ERLP \\ \hline \hline
                       100000 &   349.82 &    5.69 &  230.97 &      74 &            5 &    264.2 \\
                       200000 &  1784.52 &   14.37 &  198.83 &     276 &            8 &    551.2  \\
                       300000 &  3986.39 &   22.52 &  350.85 &     407 &           12 &    685.76 \\
                       400000 &  8040.18 &   29.58 &  847.11 &     770 &           13 &   1183.4 \\
                       500000 & 10372.00 &   39.87 &  643.73 &     885 &           15 &   1782.8 \\
                       600000 &        - &   46.56 &  759.13 &     730 &           14 &   1365.6 \\
                       700000 &        - &   55.49 & 2279.88 &     462 &           12 &    970.8 \\
                       800000 &        - &   66.09 &  979.85 &     389 &            9 &    713.8 \\
                       900000 &        - &   75.76 & 3081.46 &     284 &            3 &    454.8 \\
                      1000000 &        - &   87.71 & 1861.16 &      51 &            1 &    126.3 \\  \hline
        \end{tabular}
    \end{center}
\end{table}

\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of maximum memory consumption for artificial data sets.}
        \label{tab3}
        \begin{tabular}{|l||r|r|r|r|r|r|r|} \hline 
            & \multicolumn{6}{|c|}{Memory (MB)} \\ \hline
            Sample size ($m$) & naive LP & LPBoost & ERLP & NZDD-LP & NZDD-LPBoost & NZDD-ERLP \\ \hline \hline
                       100000 &      271 &     207 &  478 &     179 &           52 &       358 \\
                       200000 &      535 &     409 &  402 &     270 &           72 &       518 \\
                       300000 &      809 &     584 &  597 &     324 &           91 &       691 \\
                       400000 &     1070 &     785 & 1048 &     385 &          105 &       765 \\
                       500000 &     1355 &     973 &  979 &     389 &          108 &       807 \\
                       600000 &        - &    1182 & 1160 &     384 &          108 &       814 \\
                       700000 &        - &    1408 & 1934 &     346 &          100 &       749 \\
                       800000 &        - &    1515 & 1579 &     287 &           84 &       652 \\
                       900000 &        - &    1829 & 2609 &     227 &           66 &       489 \\
                      1000000 &        - &    1935 & 1985 &     125 &           40 &       253 \\  \hline
        \end{tabular}
    \end{center}
\end{table}
\fi  
  
  
\subsection{Experiments on Real Data Sets}

\begin{figure*}[htbp]
    \begin{center}
        \includegraphics[width=15cm,height=8cm,keepaspectratio]{figs/plot_time_boosting.pdf}
        \includegraphics[width=15cm,height=8cm,keepaspectratio]{figs/plot_memory_boosting.pdf}
        \caption{Comparison of computation times and maximum memory consumption 
        for real data sets. 
        The y-axes are  plotted in the logarithmic scale.}
        \end{center}
    
\end{figure*}

\iffalse
\begin{table}[htbp]
            \begin{center}
                \caption{Comparison of computation times for real data sets.}
                \label{tab6}
                \begin{tabular}{|l||r|r|r||r|r|r|} \hline
                    &\multicolumn{6}{|c|}{Computation time(sec.)} \\ \hline
                    data set   &     naive LP &    LPBoost &      ERLP & Comp. LP & Comp. LPB & Comp. ERLP \\ \hline
                    a9a        &     $330.25$ &     $3.17$ &  $269.87$ &   $9.24$ &   $8.41$ &   $104.67$ \\
                    art-100000 &   $2,504.59$ &     $5.64$ &$1,091.00$ &  $88.88$ &   $4.39$ &  $198.69$ \\
                    covtype    &  $19,156.21$ &     $8.69$ &$3,890.03$ &   $0.04$ &   $0.09$ &    $0.42$ \\
                    real-sim   &   $2,082.76$ &   $888.95$ &$2,021.37$ &   $0.26$ & $160.60$ &    $0.26$ \\
                    w8a        &     $252.26$ &     $6.14$ &   $51.44$ &   $3.18$ &  $45.62$ &    $6.75$ \\
                    ijcnn12    &              &            &           &      $0$ &          &           \\
                    HIGGS      &              &            &           &   $0.04$ &          &           \\ \hline
                \end{tabular}
    \end{center}
\end{table}

\begin{table}[htbp]
            \begin{center}
                \caption{Comparison of maximum memory consumption for real data sets.}
                \label{tab7}
                \begin{tabular}{|l||r|r|r||r|r|r|} \hline
                    &\multicolumn{6}{|c|}{Maximum memory consumption(megabytes)} \\ \hline
                    data set   & naive LP & LPBoost &   ERLP & Comp. LP & Comp. LPB& Comp. ERLP \\ \hline
                    a9a        &  $1,198$ &    $89$ &  $297$ &     $83$ &   $79$ &   $122$ \\
                    art-100000 &    $991$ &   $219$ &  $688$ &    $175$ &   $52$ &   $292$ \\
                   % covtype    & $10,326$ & $1,142$ &$2,239$ &     $13$ &   $12$ &    $14$ \\
                    real-sim   &$324,995$ &   $254$ &  $620$ &     $37$ & $1432$ &    $22$ \\
                    w8a        &  $4,083$ &   $108$ &  $242$ &    $125$ &   $46$ &   $122$ \\
                    ijcnn12    &          &         &        &     $10$ &        &         \\
                    HIGGS      &          &         &        &     $12$ &        &         \\\hline
                \end{tabular}
            \end{center}
\end{table}
\fi


%test error 
\begin{table}[htbp]
    \begin{center}
        \caption{Test error rates for real data sets}
        \label{tab8}
        \begin{tabular}{|c||c|c|c|} \hline
            data set   & \multicolumn{3}{|c|}{Test error rates} \\ \cline{2-5}
                       & LPBoost & Comp. LP & Comp. ERLP \\ \hline \hline
            a9a        & $0.174$ &  $0.159$ & $0.157$ \\
            art-100000 & $0.000$ & $0.0004$ & $0.004$ \\
%                    covtype    & $0.488$ &      $1$ & $0.488$ \\
            real-sim   & $0.179$ &  $0.169$ & $0.532$ \\
            w8a        & $0.030$ &  $0.030$ & $0.029$ \\
            ijcnn12    &         &   $0.09$ &         \\ \hline
        \end{tabular}
    \end{center}
\end{table}


\subsection{Set covering?}


\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of computation times for real data sets.}
        % \label{tab}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{Computation time(sec.)} \\ \hline
            data set   &     naive IP & Comp. IP \\ \hline
            chess      &     $0.15$   &      $0.1$  \\
            connect    &     $7.26$   &     $3.82$  \\
            mushroom   &     $0.15$   &     $0.01$  \\
            pumsb      &     $14.5$   &    $14.23$  \\
            pumsb\_star&    $10.89$   &     $8.64$  \\
            kosarak    &    $11.83$   &    $14.01$  \\
            retail     &     $1.11$   &     $1.86$  \\
            accidents  &    $72.22$   &   $114.66$  \\ \hline
        \end{tabular}
    \end{center}
  \end{table}

  \begin{table}[htbp]
    \begin{center}
        \caption{Comparison of maximum memory consumption for real data sets.}
        % \label{tab}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{Maximum memory(megabytes)} \\ \hline
            data set   &     naive IP & Comp. IP \\ \hline
            chess      &       $26$   &       $22$  \\
            connect    &      $656$   &      $192$  \\
            mushroom   &       $36$   &       $13$  \\
            pumsb      &      $504$   &      $545$  \\
            pumsb\_star&      $348$   &      $360$  \\
            kosarak    &     $1277$   &     $1091$  \\
            retail     &      $151$   &      $155$  \\
            accidents  &     $2422$   &     $2603$  \\ \hline
        \end{tabular}
    \end{center}
  \end{table}
  



==> experiments_old2.tex <==
\section{Experiments}
\label{sec:experiments}
We show preliminary experimental results on artificial and real large data sets. 
The tasks are, the set covering problem (see, e.g., \citet{williamson-shmoys:book11}), an integer programming task, and 
the $1$-norm regularized soft margin optimization, a linear programming task, as in (\ref{prob:softmargin_primal}).
Our experiments are conducted on a server with 2.60 GHz Intel Xeon Gold 6124 CPUs and 314GB memory.
We use Gurobi optimizer 9.01
\footnote{Gurobi Optimization, Inc.,\url{http://www.gurobi.com} }, an state-of-the-art commercial LP solver.
To obtain NZDD representations of data sets, we apply the procedure described in Section \ref{sec:construction}.
The details of preprocessing of data sets and NZDD representations are shown in Appendix.

\subsection{Integer programming(IP)}
First, we apply our extended formulation (\ref{prob:lin_const_opt}) to the set covering problem~\citep{}, an integer programming tasks.
We use real datasets tested in the paper of \citet{cormode-etal:cikm10}, 
which are found in Goethal's web page~\citep{goethals:web} and 
in the UCI Machine Learning Repository~\citep{uci-ml}. 
Here, our intention on these experiments is not to compare the state-of-the-art set covering solvers (e.g.,\citet{cormode-etal:cikm10}),
but to confirm advantages to off-the-shelf IP solvers on general IP data sets. 
So, we apply the Gruobi optimizer to the standard IP formulation of the set covering 
and our extended formulation for the set covering, respectively.
The results are summarized in Figure~\ref{fig:setcover}. 
Our method consistently improve both computation time and often reduce memory usage. 

\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_time_setcover.pdf}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_memory_setcover.pdf}
        \caption{Comparison of computation times and maximum memory consumption 
        for real datasets of set covering problems. The y-axes are shown in the logarithmic scale.}
        \label{fig:setcover}   
    \end{center} 
\end{figure}


\iffalse
\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of computation times for real data sets.}
        \label{tab10}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{Computation time(sec.)} \\ \hline
            data set    & naive LP & proposed\\ \hline
            chess       &     $0.15$ & $0.1$ \\
            connect     &     $7.26$ & $3.82$ \\
            mushroom    &     $0.15$ & $0.01$  \\
            pumsb       &     $14.5$ & $14.23$  \\
            pumsb\_star &    $10.89$ & $8.64$ \\ \hline
        \end{tabular}
    \end{center}
\end{table}

\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of maximum memory consumption for real data sets.}
        \label{tab9}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{memory(MB)} \\ \hline
            data set    & naive LP & proposed\\ \hline
            chess       &     $26$ & $22$ \\
            connect     &    $656$ & $192$ \\
            mushroom    &     $35$ & $13$  \\
            pumsb       &    $504$ & $544$  \\
            pumsb\_star &    $348$ & $359$ \\ \hline
        \end{tabular}
    \end{center}
\end{table}
\fi




\subsection{$1$-norm soft margin optimization}

We compare the following methods.
\begin{description}
    \item[LP] 
    We naively apply the LP solver to solve problem (\ref{prob:softmargin_primal}).
    \item [LPBoost] 
    LPBoost\citep{demiriz-etal:ml02} is a standard method for solving (\ref{prob:softmargin_primal}).
    LPBoost is a "column-generation" type medhod, i.e., 
    it solves the dual subproblems of (\ref{prob:softmargin_primal}) iteratively by adding constraints.
    \item[Our method]...
\end{description}



\subsubsection{Experiments on Artificial Data Sets}
We use a class of artificial data sets that have small NZDD representations when the samples are large. 
Our artificial data sets are made by a simple linear threshold function over the domain $\{0,1\}^n$ for some positive integer $n$.
First, we choose $m$ instances in $\{0,1\}^n$ uniformly randomly without repetition. 
Then we consider the following linear threshold function $f(\vecx)=\sign(\sum_{j=1}^k x_j - r+ 1/2)$, 
where $k$ and $r$ are positive integers such that $1\leq r\leq k\leq n$).
That is, $f(x)=1$ if and only if at least $r$ of the first $k$ components are $1$. We call this $r$-of-$k$ threshold function.
Each label of the instance $\vecx\in\{0,1\}^n$ is labeled by $f(\vecx)$. It can be easily shown that 
the whole labeled $2^n$ instances of $f$ is represented by an NZDD (or ZDD) of size $O(kr)$, 
which is exponentially small w.r.t. the sample size $m=2^n$. 
We fix $n=20$, $k=10$ and $r=5$. Then we use $m \in \{1*10^5,2*10^5...,10^6\}$.

\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_time_artificial.pdf}
        \includegraphics[width=7cm,height=6cm,keepaspectratio]{figs/plot_memory_artificial.pdf}
        \caption{Comparison of computation times and maximum memory consumption 
        for artificial data sets. 
        Results for naive LP w.r.t. $m\geq 6*10^5$ are omitted since it takes more than $1$ day.}
        \end{center}
    
\end{figure}

\iffalse
\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of computation times for artificial data sets.}
        \label{tab2}
        \begin{tabular}{|l||r|r|r|r|r|r|r|} \hline 
            & \multicolumn{6}{|c|}{Computation time (sec.)} \\ \hline
            Sample size ($m$) & naive LP & LPBoost &   ERLP & NZDD-LP & NZDD-LPBoost & NZDD-ERLP \\ \hline \hline
                       100000 &   349.82 &    5.69 &  230.97 &      74 &            5 &    264.2 \\
                       200000 &  1784.52 &   14.37 &  198.83 &     276 &            8 &    551.2  \\
                       300000 &  3986.39 &   22.52 &  350.85 &     407 &           12 &    685.76 \\
                       400000 &  8040.18 &   29.58 &  847.11 &     770 &           13 &   1183.4 \\
                       500000 & 10372.00 &   39.87 &  643.73 &     885 &           15 &   1782.8 \\
                       600000 &        - &   46.56 &  759.13 &     730 &           14 &   1365.6 \\
                       700000 &        - &   55.49 & 2279.88 &     462 &           12 &    970.8 \\
                       800000 &        - &   66.09 &  979.85 &     389 &            9 &    713.8 \\
                       900000 &        - &   75.76 & 3081.46 &     284 &            3 &    454.8 \\
                      1000000 &        - &   87.71 & 1861.16 &      51 &            1 &    126.3 \\  \hline
        \end{tabular}
    \end{center}
\end{table}

\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of maximum memory consumption for artificial data sets.}
        \label{tab3}
        \begin{tabular}{|l||r|r|r|r|r|r|r|} \hline 
            & \multicolumn{6}{|c|}{Memory (MB)} \\ \hline
            Sample size ($m$) & naive LP & LPBoost & ERLP & NZDD-LP & NZDD-LPBoost & NZDD-ERLP \\ \hline \hline
                       100000 &      271 &     207 &  478 &     179 &           52 &       358 \\
                       200000 &      535 &     409 &  402 &     270 &           72 &       518 \\
                       300000 &      809 &     584 &  597 &     324 &           91 &       691 \\
                       400000 &     1070 &     785 & 1048 &     385 &          105 &       765 \\
                       500000 &     1355 &     973 &  979 &     389 &          108 &       807 \\
                       600000 &        - &    1182 & 1160 &     384 &          108 &       814 \\
                       700000 &        - &    1408 & 1934 &     346 &          100 &       749 \\
                       800000 &        - &    1515 & 1579 &     287 &           84 &       652 \\
                       900000 &        - &    1829 & 2609 &     227 &           66 &       489 \\
                      1000000 &        - &    1935 & 1985 &     125 &           40 &       253 \\  \hline
        \end{tabular}
    \end{center}
\end{table}
\fi  
  
  
\subsection{Experiments on Real Data Sets}

\begin{figure*}[htbp]
    \begin{center}
        \includegraphics[width=15cm,height=8cm,keepaspectratio]{figs/plot_time_boosting.pdf}
        \includegraphics[width=15cm,height=8cm,keepaspectratio]{figs/plot_memory_boosting.pdf}
        \caption{Comparison of computation times and maximum memory consumption 
        for real data sets. 
        The y-axes are  plotted in the logarithmic scale.}
        \end{center}
    
\end{figure*}

\iffalse
\begin{table}[htbp]
            \begin{center}
                \caption{Comparison of computation times for real data sets.}
                \label{tab6}
                \begin{tabular}{|l||r|r|r||r|r|r|} \hline
                    &\multicolumn{6}{|c|}{Computation time(sec.)} \\ \hline
                    data set   &     naive LP &    LPBoost &      ERLP & Comp. LP & Comp. LPB & Comp. ERLP \\ \hline
                    a9a        &     $330.25$ &     $3.17$ &  $269.87$ &   $9.24$ &   $8.41$ &   $104.67$ \\
                    art-100000 &   $2,504.59$ &     $5.64$ &$1,091.00$ &  $88.88$ &   $4.39$ &  $198.69$ \\
                    covtype    &  $19,156.21$ &     $8.69$ &$3,890.03$ &   $0.04$ &   $0.09$ &    $0.42$ \\
                    real-sim   &   $2,082.76$ &   $888.95$ &$2,021.37$ &   $0.26$ & $160.60$ &    $0.26$ \\
                    w8a        &     $252.26$ &     $6.14$ &   $51.44$ &   $3.18$ &  $45.62$ &    $6.75$ \\
                    ijcnn12    &              &            &           &      $0$ &          &           \\
                    HIGGS      &              &            &           &   $0.04$ &          &           \\ \hline
                \end{tabular}
    \end{center}
\end{table}

\begin{table}[htbp]
            \begin{center}
                \caption{Comparison of maximum memory consumption for real data sets.}
                \label{tab7}
                \begin{tabular}{|l||r|r|r||r|r|r|} \hline
                    &\multicolumn{6}{|c|}{Maximum memory consumption(megabytes)} \\ \hline
                    data set   & naive LP & LPBoost &   ERLP & Comp. LP & Comp. LPB& Comp. ERLP \\ \hline
                    a9a        &  $1,198$ &    $89$ &  $297$ &     $83$ &   $79$ &   $122$ \\
                    art-100000 &    $991$ &   $219$ &  $688$ &    $175$ &   $52$ &   $292$ \\
                   % covtype    & $10,326$ & $1,142$ &$2,239$ &     $13$ &   $12$ &    $14$ \\
                    real-sim   &$324,995$ &   $254$ &  $620$ &     $37$ & $1432$ &    $22$ \\
                    w8a        &  $4,083$ &   $108$ &  $242$ &    $125$ &   $46$ &   $122$ \\
                    ijcnn12    &          &         &        &     $10$ &        &         \\
                    HIGGS      &          &         &        &     $12$ &        &         \\\hline
                \end{tabular}
            \end{center}
\end{table}
\fi


%test error 
\begin{table}[htbp]
    \begin{center}
        \caption{Test error rates for real data sets}
        \label{tab8}
        \begin{tabular}{|c||c|c|c|} \hline
            data set   & \multicolumn{3}{|c|}{Test error rates} \\ \cline{2-5}
                       & LPBoost & Comp. LP & Comp. ERLP \\ \hline \hline
            a9a        & $0.174$ &  $0.159$ & $0.157$ \\
            art-100000 & $0.000$ & $0.0004$ & $0.004$ \\
%                    covtype    & $0.488$ &      $1$ & $0.488$ \\
            real-sim   & $0.179$ &  $0.169$ & $0.532$ \\
            w8a        & $0.030$ &  $0.030$ & $0.029$ \\
            ijcnn12    &         &   $0.09$ &         \\ \hline
        \end{tabular}
    \end{center}
\end{table}


\subsection{Set covering?}


\begin{table}[htbp]
    \begin{center}
        \caption{Comparison of computation times for real data sets.}
        % \label{tab}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{Computation time(sec.)} \\ \hline
            data set   &     naive IP & Comp. IP \\ \hline
            chess      &     $0.15$   &      $0.1$  \\
            connect    &     $7.26$   &     $3.82$  \\
            mushroom   &     $0.15$   &     $0.01$  \\
            pumsb      &     $14.5$   &    $14.23$  \\
            pumsb\_star&    $10.89$   &     $8.64$  \\
            kosarak    &    $11.83$   &    $14.01$  \\
            retail     &     $1.11$   &     $1.86$  \\
            accidents  &    $72.22$   &   $114.66$  \\ \hline
        \end{tabular}
    \end{center}
  \end{table}

  \begin{table}[htbp]
    \begin{center}
        \caption{Comparison of maximum memory consumption for real data sets.}
        % \label{tab}
        \begin{tabular}{|l||r|r|} \hline
            &\multicolumn{2}{|c|}{Maximum memory(megabytes)} \\ \hline
            data set   &     naive IP & Comp. IP \\ \hline
            chess      &       $26$   &       $22$  \\
            connect    &      $656$   &      $192$  \\
            mushroom   &       $36$   &       $13$  \\
            pumsb      &      $504$   &      $545$  \\
            pumsb\_star&      $348$   &      $360$  \\
            kosarak    &     $1277$   &     $1091$  \\
            retail     &      $151$   &      $155$  \\
            accidents  &     $2422$   &     $2603$  \\ \hline
        \end{tabular}
    \end{center}
  \end{table}
  



==> symbol_old.tex <==
%
% symbol.tex
%

\newcommand{\hsigma}{\widehat\sigma}
\newcommand{\convhull}{\mathcal{H}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\dom}{\mathcal{X}} %domain of interest
\newcommand{\calP}{\mathcal{P}}
\newcommand{\Natural}{\mathbb{N}} % 
\newcommand{\Real}{\mathbb{R}} % Eucledian space
\newcommand{\Prob}{\mathcal{P}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\Hyp}{\mathcal{H}}
\newcommand{\WH}{\mathcal{W}}
\newcommand{\EX}{\mathrm{EX}}
\newcommand{\filtEX}{\mathrm{FiltEX}}
\newcommand{\HSelect}{\mathrm{HSelect}}
\newcommand{\WL}{\mathrm{WL}}
%\newcommand{\breg}{D}
\newcommand{\vecx}{\bm{x}}
\newcommand{\vecy}{\bm{y}}
\newcommand{\vecw}{\bm{w}}
\newcommand{\vecz}{\bm{z}}
\newcommand{\vecg}{\bm{g}}
\newcommand{\veca}{\bm{a}}
\newcommand{\vecb}{\bm{b}}
\newcommand{\vecs}{\bm{s}}
\newcommand{\vecd}{\mbox{\boldmath $d$}}
\newcommand{\vecell}{\mbox{\boldmath $\ell$}}
\newcommand{\vecsigma}{\bm{\sigma}}
\newcommand{\vecpi}{\bm{\pi}}
\newcommand{\veceta}{\bm{\eta}}
%\newcommand{\vecv}{\mbox{\boldmath $v$}}
\newcommand{\vecxi}{\bm{\xi}}
\newcommand{\vece}{\mbox{\boldmath $e$}}
\newcommand{\vecB}{\mbox{\boldmath $B$}}
\newcommand{\vecD}{\mbox{\boldmath $D$}}
\newcommand{\vecI}{\mbox{\boldmath $I$}}
\newcommand{\idx}{\mathrm{idx}}
%\newcommand{\vecpi}{\mbox{\boldmath $\pi$}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\vecG}{\mbox{\boldmath $G$}}
\newcommand{\vecF}{\mbox{\boldmath $F$}}
\newcommand{\tvecu}{\tilde{\mbox{\boldmath $u$}}}
\newcommand{\tvecw}{\tilde{\mbox{\boldmath $w$}}}
\newcommand{\tvecx}{\tilde{\mbox{\boldmath $x$}}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\haty}{\hat{y}}
\newcommand{\vecf}{\mbox{\boldmath $f$}}
\newcommand{\vectheta}{\mbox{\boldmath $\theta$}}
\newcommand{\vecTheta}{\bm{\Theta}}
\newcommand{\vecGamma}{\bm{\Gamma}}
\newcommand{\vecalpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\vecbeta}{\bm{\beta}}
\newcommand{\vectau}{\mbox{\boldmath $\tau$}}
\newcommand{\tgamma}{\tilde\gamma}
\newcommand{\vecgamma}{\bm{\gamma}}
\newcommand{\vectgamma}{\bm{\tilde\gamma}}
\newcommand{\veclambda}{\bm{\lambda}}
\newcommand{\vecu}{\mbox{\boldmath $u$}}
\newcommand{\vecv}{\mbox{\boldmath $v$}}
\newcommand{\vecp}{\boldsymbol{p}}
\newcommand{\vecq}{\mbox{\boldmath $q$}}
\newcommand{\vecr}{\bm{r}}
\newcommand{\vecc}{\bm{c}}
\newcommand{\matA}{\bm{A}}

\newcommand{\fp}{\mathrm{fp}}
\newcommand{\fn}{\mathrm{fn}}
\newcommand{\ouralgorithm}{{Follow the Reguralized Leader}~}
\newcommand{\ouralg}{{FTRL}~}
\newcommand{\Ouralg}{PUMMA~}%{Modified ROMMA~}

\newcommand{\bn}{\Delta_2} % binary entropy
\newcommand{\psimp}{\mathcal{P}} %
\newcommand{\hatgamma}{\hat{\gamma}}
%\newcommand{\example}{\langle x,f(x) \rangle}
\newcommand{\indctr}[1]{I(#1)}
\newcommand{\CLASS}{\mathcal{C}}
\newcommand{\VC}{\mathrm{VC}}

\newcommand{\reg}{\mathcal{R}}
\newcommand{\breg}{D}

\newcommand{\filtex}{\mathrm{GenD_t}}
\newcommand{\gensamp}{\mathrm{GenSample}}



\newcommand{\half}{\frac{1}{2}}
\newcommand{\eps}{\varepsilon}

\newcommand{\hp}{\hat{p}}
\newcommand{\hmup}{\hat{\mu}[+]}
\newcommand{\hmun}{\hat{\mu}[-]}
\newcommand{\hgp}{\hat{\gamma}[+]}
\newcommand{\hgn}{\hat{\gamma}[-]}
\newcommand{\gain}{\Delta}
\newcommand{\hgain}{\hat{\Delta}}
\newcommand{\vecdelta}{\bm{\delta}}
\newcommand{\vecLambda}{\bm{\Lambda}}
\newcommand{\vecX}{\bm{X}}
\newcommand{\vecW}{\bm{W}}
\newcommand{\tildeO}{\Tilde{O}}
\newcommand{\permset}{S}
\newcommand{\base}{\bm{B}}
\newcommand{\calC}{\mathcal{C}}




%
%
%
\def\ceil#1{%
\left\lceil #1 \right\rceil}

\def\defeq{%
\stackrel{\mathrm{def}}{=}}

\def\floor#1{%
\lfloor #1 \rfloor}

\def\myhang{%
    \par\noindent\hangindent20pt\hskip20pt}
\def\nitem#1{%
    \par\noindent\hangindent40pt
    \hskip40pt\llap{#1~}}


\newcommand{\E}{\mathbf{E}}
\newcommand{\mynote}[1]{\textbf{#1}}



==> table/softmargin-real-time.tex <==
\begin{tabular}{lrrrrrr} \hline
    \toprule
    data set   &     naive LP &    LPBoost &      ERLP & Comp. LP & Comp. LPB & Comp. ERLP \\
    \midrule
    a9a        &     $330.25$ &     $3.17$ &  $269.87$ &   $9.24$ &   $8.41$ &   $104.67$ \\
    art-100000 &   $2,504.59$ &     $5.64$ &$1,091.00$ &  $88.88$ &   $4.39$ &  $198.69$ \\
    covtype    &  $19,156.21$ &     $8.69$ &$3,890.03$ &   $0.04$ &   $0.09$ &    $0.42$ \\
    real-sim   &   $2,082.76$ &   $888.95$ &$2,021.37$ &   $0.26$ & $160.60$ &    $0.26$ \\
    w8a        &     $252.26$ &     $6.14$ &   $51.44$ &   $3.18$ &  $45.62$ &    $6.75$ \\
    \bottomrule
\end{tabular}


